Ming-UniAudio: Speech LLM for Joint Understanding, Generation and Editing with Unified Representation

Existing speech models suffer from competing requirements on token representations by understanding and generation tasks. This discrepancy in representation prevents speech language models from performing instruction-based free-form editing. To solve this challenge, we introduce a novel framework that unifies speech understanding, generation, and editing. The core of our unified model is a unified continuous speech tokenizer MingTok-Audio, the first continuous tokenizer to effectively integrate semantic and acoustic features, which makes it suitable for both understanding and generation tasks. Based on this unified continuous audio tokenizer, we developed the speech language model Ming-UniAudio, which achieved a balance between generation and understanding capabilities. Ming-UniAudio sets new state-of-the-art (SOTA) records on 8 out of 12 metrics on the ContextASR benchmark. Notably, for Chinese voice cloning, it achieves a highly competitive Seed-TTS-WER of 0.95. Leveraging this foundational model, we further trained a dedicated speech editing model Ming-UniAudio-Edit, the first speech language model that enables universal, free-form speech editing guided solely by natural language instructions, handling both semantic and acoustic modifications without timestamp condition. To rigorously assess the editing capability and establish a foundation for future research, we introduce Ming-Freeform-Audio-Edit, the first comprehensive benchmark tailored for instruction-based free-form speech editing, featuring diverse scenarios and evaluation dimensions spanning semantic correctness, acoustic quality, and instruction alignment. We open-sourced the continuous audio tokenizer, the unified foundational model, and the free-form instruction-based editing model to facilitate the development of unified audio understanding, generation, and manipulation.

==> sections/5-3-sft-task-semantic.tex <==
\subsection{Semantic Tasks}
For semantic editing tasks, we adopt an instruction-following format allowing us to effectively leverage the pre-trained model's ability to comprehend and execute instructions. The data is structured as follows:

\[
    \mathtt{SourceSpeech}_{z_{\mathtt{uni}}} + \mathtt{Instruction}_{\mathtt{text}}  \rightarrow \mathtt{CoT}_{\mathtt{text}} + \mathtt{TargetSpeech}_{z_{\mathtt{latent}}}
\]
We introduced several key innovations to achieve free-form instruction following:
\begin{itemize}

\item  \textbf{CoT for edited text:} To begin with, we explicitly incorporate a chain-of-thought (CoT) \citep{wei2023chainofthoughtpromptingelicitsreasoning} output, which represents the textual content of the edited speech. CoT has been proven to be a highly effective technique in LLM, and its inclusion here significantly improves the pronunciation and instruction-following quality of the output audio.
\item  \textbf{Mask for edited region text:} Furthermore, we use a special [MASK] token to denote the positions corresponding to the regions to be edited within the CoT text. This enhances the model's positional awareness of the editing regions. Subsequent experiments demonstrate that this modification is effective in improving the editing accuracy of the output audio.
\item  \textbf{Audio loss weighting:} In addition, during the training process, we apply a weighted loss to the edited regions of the output speech. This strengthens the model's ability to learn from these specific segments. For non-edited regions, the model can directly copy information from the input speech, which reduces the learning difficulty.
\item  \textbf{Instruction-augument:} Another key aspect is our effort to better align with the behavior of the real world user. We leverage a powerful pre-trained text LLM model to augment the instructions in our training data, which also enhances the model's generalization capabilities to some extent.
\item  \textbf{Novel Data Strategy:} Finally, we dedicate a significant effort to data construction to ensure the quality of input and output speech pairs. A detailed discussion of this process can be found in Section \ref{sec:instruction data}

\end{itemize}


\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/speech_edit_data.png}
    \caption{Speech Edit Data Construction Method}
    \label{fig:speech_edit_data}
\end{figure}


